DAVIO: Dense Monocular-Inertial SLAM with Feed-Forward Initialization and Pose-Conditioned Mapping

A camera and an IMU are the minimal sensor setup for metric localization and dense mapping, yet classical visual--inertial filters must wait for parallax before they start and then retain only sparse landmarks. Feed-forward geometry models, in contrast, predict dense structure from a few images but provide neither metric scale nor gravity. We present DAVIO, which uses a single multi-view depth model, Depth Anything~3, for both start-up and mapping. At start-up, a five-image window and preintegrated IMU measurements form a feature-free linear system. Its robust, conditioning-checked solution bootstraps a VIO filter through buffered replay. During tracking, the filter's metric poses condition the depth model. Residual scale is corrected only along viewing rays, which preserves the metric camera baselines, and a gravity-preserving submap graph with drift-gated revisits refines the map. On EuRoC, DAVIO starts markedly earlier, reduces the localization error, and maps more accurately than SOTA feed-forward mappers given identical poses. On building-scale ORI sequences, DAVIO is on bar or better than SOTA mappers on the same odometry, and degrades far less when GT poses are replaced by real odometry. We release the code of DAVIO, a real-time dense metric SLAM system, to the community.

==> tables/tab_cmp_euroc_map.tex <==
% generated by paper/submission/build_comparison_tables.py from assets.json
\begin{table}[t]\centering\footnotesize
\caption{EuRoC Vicon-room reconstruction against the Leica scans: F@10 and mean map-to-reference distance (m) under the trajectory's rigid alignment and frozen support. All three maps use the same OpenVINS trajectory and DA3-Base at 4\,cm density; ScaRF's released mapper runs offline. MASt3R-Fusion and VGGT-SLAM2 were run on the machine-hall sequences only (no reference scan). Best in bold.}\label{tab:cmp_euroc_map}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lcccccc}\toprule
 & \multicolumn{2}{c}{DAVIO online} & \multicolumn{2}{c}{DAVIO mapper offline} & \multicolumn{2}{c}{ScaRF mapper}\\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
Seq. & F@10 & Mean & F@10 & Mean & F@10 & Mean\\\midrule
V1\_01 & 0.64 & \textbf{0.125} & \textbf{0.68} & 0.132 & 0.42 & 0.242\\
V1\_02 & \textbf{0.68} & \textbf{0.115} & 0.62 & 0.163 & 0.49 & 0.216\\
V1\_03 & \textbf{0.52} & 0.205 & \textbf{0.52} & \textbf{0.201} & 0.41 & 0.288\\
V2\_01 & \textbf{0.61} & \textbf{0.167} & 0.55 & 0.205 & 0.48 & 0.210\\
V2\_02 & \textbf{0.55} & \textbf{0.177} & 0.53 & 0.204 & 0.35 & 0.290\\
V2\_03 & 0.48 & \textbf{0.188} & 0.41 & 0.255 & \textbf{0.49} & 0.211\\
\midrule
Median & \textbf{0.58} & \textbf{0.172} & 0.54 & 0.203 & 0.45 & 0.229\\
\bottomrule
\end{tabular}
\end{table}


==> tables/tab_cmp_euroc_traj.tex <==
% generated by paper/submission/build_comparison_tables.py from assets.json
\begin{table*}[t]\centering\footnotesize
\caption{EuRoC trajectory error: ATE (m) after one rigid SE(3) alignment, OpenVINS reference. OpenVINS: median of three mapping-disabled runs; DAVIO: raw VIO and final corrected trajectory; ORB-SLAM3, MASt3R-Fusion and VGGT-SLAM2: released code, median of three runs (ORB-SLAM3 range 0.036--0.091, 0.049--0.055, 0.055--0.069\,m; the two learned systems repeat exactly). Poses scored: ORB-SLAM3 74--82\,\% of the frames (largest map), MASt3R-Fusion 49\,\% (every second image), VGGT-SLAM2 4--7\,\% (keyframes). $^\dagger$Monocular; one global Sim(3) scale fitted to the reference first. Best in bold, raw VIO and keyframes excluded.}\label{tab:cmp_euroc_traj}
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lccccccc}\toprule
 & OpenVINS & \multicolumn{2}{c}{DAVIO} & ORB-SLAM3 & \multicolumn{2}{c}{MASt3R-Fusion} & VGGT-SLAM2$^\dagger$\\\cmidrule(lr){3-4}\cmidrule(lr){6-7}
Seq. & native & raw & final & mono-inertial & real-time & keyframes & keyframes\\\midrule
MH\_01 & 0.099 & 0.126 & 0.065 & \textbf{0.058} & 0.419 & 0.344 & 0.188\\
MH\_03 & 0.158 & 0.158 & 0.101 & \textbf{0.053} & 0.447 & 0.424 & 0.337\\
MH\_05 & 0.281 & 0.281 & 0.200 & \textbf{0.060} & 0.555 & 0.513 & 0.989\\
\bottomrule
\end{tabular}
\end{table*}


==> tables/tab_cmp_ori.tex <==
% generated by paper/submission/build_comparison_tables.py from assets.json
\begin{table}[t]\centering\footnotesize
\caption{ORI R01--R05 reconstruction, medians over the five sequences. Global: map-to-reference distance under the trajectory's rigid alignment (2\,cm export, frozen support). Chunks: the released ScaRF evaluator (10\,m chunks, Sim(3)+ICP, 3\,cm). $^\dagger$Monocular; poses and map scaled by one global Sim(3) fit to the reference. Best measured value in bold. Published rows (ScaRF-SLAM with DA3-Giant) are quoted, not rerun.}\label{tab:cmp_ori}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lccccc}\toprule
 & \multicolumn{2}{c}{Global} & \multicolumn{3}{c}{10\,m chunks}\\\cmidrule(lr){2-3}\cmidrule(lr){4-6}
System & Mean & F@10 & Err. & P@3 & R@3\\
 & (m) & & (m) & (\%) & (\%)\\\midrule
\multicolumn{6}{l}{\emph{Measured, DAVIO's OpenVINS trajectory, DA3}}\\
\quad DAVIO online (Base) & 0.080 & 0.75 & 0.044 & 60.8 & 38.8\\
\quad DAVIO online (Large) & \textbf{0.061} & \textbf{0.81} & \textbf{0.033} & \textbf{71.9} & 38.3\\
\quad DAVIO mapper, offline & 0.087 & 0.78 & 0.040 & 61.9 & 52.9\\
\quad ScaRF mapper, offline & 0.084 & 0.69 & 0.043 & 61.6 & 43.9\\
\midrule
\multicolumn{6}{l}{\emph{Measured, own trajectory}}\\
\quad MASt3R-Fusion & 0.194 & 0.67 & 0.123 & 49.6 & \textbf{61.4}\\
\quad VGGT-SLAM2$^\dagger$ & 0.161 & 0.50 & 0.110 & 34.0 & 14.3\\
\midrule
\multicolumn{6}{l}{\emph{Published by the ScaRF-SLAM authors}}\\
\quad ScaRF-SLAM & -- & -- & 0.020 & 81.3 & 55.8\\
\quad MASt3R-Fusion & -- & -- & 0.058 & 54.4 & 41.8\\
\quad VGGT-SLAM2 & -- & -- & 0.169 & 23.8 & 21.9\\
\bottomrule
\end{tabular}
\end{table}


==> tables/tab_cmp_ori_seq.tex <==
% generated by paper/submission/build_comparison_tables.py from assets.json
\begin{table}[t]\centering\footnotesize
\caption{ORI per sequence. DAVIO online and ScaRF's mapper use the same OpenVINS trajectory (DA3-Base); MASt3R-Fusion and VGGT-SLAM2 use their own trajectories. Published values (publ.) are the ScaRF-SLAM authors' Table III. $^\dagger$Scale-corrected by one global Sim(3) fit. Best measured value per column in bold.}\label{tab:cmp_ori_seq}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lcccccc}\toprule
System & R01 & R02 & R03 & R04 & R05 & Median\\\midrule
\multicolumn{7}{l}{\emph{Global F@10}}\\
\quad DAVIO online & \textbf{0.75} & 0.75 & \textbf{0.81} & \textbf{0.71} & 0.68 & \textbf{0.75}\\
\quad ScaRF mapper & 0.54 & \textbf{0.78} & 0.75 & 0.69 & 0.63 & 0.69\\
\quad MASt3R-Fusion & 0.71 & 0.60 & 0.67 & 0.62 & \textbf{0.75} & 0.67\\
\quad VGGT-SLAM2$^\dagger$ & 0.33 & 0.08 & 0.56 & 0.50 & 0.55 & 0.50\\
\midrule
\multicolumn{7}{l}{\emph{Chunk error (m)}}\\
\quad DAVIO online & \textbf{0.048} & 0.044 & 0.043 & \textbf{0.042} & 0.047 & 0.044\\
\quad ScaRF mapper & 0.056 & \textbf{0.038} & \textbf{0.035} & 0.045 & \textbf{0.043} & \textbf{0.043}\\
\quad MASt3R-Fusion & 0.084 & 0.123 & 0.193 & 0.149 & 0.084 & 0.123\\
\quad VGGT-SLAM2$^\dagger$ & 0.149 & 0.220 & 0.110 & 0.105 & 0.057 & 0.110\\
\quad \emph{ScaRF-SLAM (publ.)} & 0.022 & 0.021 & 0.020 & 0.020 & 0.020 & 0.020\\
\quad \emph{MASt3R-Fusion (publ.)} & 0.044 & 0.072 & 0.058 & 0.038 & 0.078 & 0.058\\
\quad \emph{VGGT-SLAM2 (publ.)} & 0.175 & 0.195 & 0.169 & 0.152 & 0.151 & 0.169\\
\midrule
\multicolumn{7}{l}{\emph{Chunk precision P@3 (\%)}}\\
\quad DAVIO online & 58.3 & 60.8 & \textbf{66.8} & \textbf{63.2} & 57.9 & 60.8\\
\quad ScaRF mapper & \textbf{61.6} & \textbf{61.9} & 65.9 & 60.8 & \textbf{60.2} & \textbf{61.6}\\
\quad MASt3R-Fusion & 49.6 & 47.0 & 54.7 & 52.9 & 49.2 & 49.6\\
\quad VGGT-SLAM2$^\dagger$ & 25.5 & 18.8 & 34.0 & 35.4 & 49.4 & 34.0\\
\quad \emph{ScaRF-SLAM (publ.)} & 81.1 & 80.4 & 81.3 & 81.6 & 82.9 & 81.3\\
\quad \emph{MASt3R-Fusion (publ.)} & 63.0 & 48.3 & 52.2 & 61.5 & 54.4 & 54.4\\
\quad \emph{VGGT-SLAM2 (publ.)} & 19.9 & 20.2 & 23.8 & 26.2 & 25.8 & 23.8\\
\midrule
\multicolumn{7}{l}{\emph{Chunk recall R@3 (\%)}}\\
\quad DAVIO online & 40.5 & 35.1 & 40.2 & 38.8 & 37.4 & 38.8\\
\quad ScaRF mapper & 44.6 & 42.5 & 46.4 & 43.9 & 43.5 & 43.9\\
\quad MASt3R-Fusion & \textbf{60.3} & \textbf{61.4} & \textbf{63.8} & \textbf{62.2} & \textbf{57.8} & \textbf{61.4}\\
\quad VGGT-SLAM2$^\dagger$ & 11.1 & 6.5 & 14.3 & 18.9 & 28.1 & 14.3\\
\quad \emph{ScaRF-SLAM (publ.)} & 57.7 & 52.0 & 55.4 & 55.8 & 56.2 & 55.8\\
\quad \emph{MASt3R-Fusion (publ.)} & 46.8 & 37.0 & 38.2 & 44.5 & 41.8 & 41.8\\
\quad \emph{VGGT-SLAM2 (publ.)} & 21.9 & 18.2 & 18.1 & 28.4 & 27.8 & 21.9\\
\bottomrule
\end{tabular}
\end{table}


==> tables/tab_ori.tex <==
% generated by paper/submission/build_assets.py from recorded artifacts
\begin{tabular}{lccccc}\toprule
 & \multicolumn{2}{c}{Global} & \multicolumn{3}{c}{10 m chunks}\\ System & Mean (m) & F@10 & Err.\ (m) & P@3 & R@3\\\midrule
Unconditioned reference & 0.219 & 0.38 & 0.157 & 20.1 & 13.9\\
DAVIO online, DA3-Base & 0.080 & 0.75 & 0.044 & 60.8 & 38.8\\
DAVIO online, DA3-Large & 0.061 & 0.81 & 0.033 & 71.9 & 38.3\\
DAVIO mapper, graph / VIO & 0.087 & 0.78 & 0.040 & 61.9 & 52.9\\
DAVIO mapper, poses fixed / VIO & 0.105 & 0.70 & 0.040 & 62.3 & 52.7\\
\quad ScaRF windows (6/1, 0.32\,s) / VIO & 0.101 & 0.69 & 0.047 & 61.4 & 44.7\\
\quad DA3-Large / VIO & 0.093 & 0.73 & 0.038 & 73.0 & 57.5\\
ScaRF mapper / VIO & 0.084 & 0.69 & 0.043 & 61.6 & 43.9\\
DAVIO mapper, graph or fixed / ref. & 0.069 & 0.88 & 0.041 & 67.8 & 54.7\\
\quad ScaRF windows / ref. & 0.069 & 0.82 & 0.048 & 62.8 & 43.5\\
ScaRF mapper / ref. & 0.040 & 0.89 & 0.029 & 70.6 & 47.7\\
ScaRF-SLAM published (DA3-Giant) & -- & -- & 0.020 & 81.3 & 55.8\\
\bottomrule\end{tabular}


==> tables/tab_ori_ablation.tex <==
% offline DAVIO mapper factors on ORI; numbers copied verbatim from tab_ori.tex /
% tab_cmp_ori.tex (medians over R01--R05)
\newcommand{\ours}{\rowcolor{gray!12}}
\newcommand{\grp}[1]{\multicolumn{6}{@{}l}{\textit{#1}}\\[1pt]}
\begin{tabular}{@{}l cc ccc@{}}
\toprule
 & \multicolumn{2}{c}{Global} & \multicolumn{3}{c}{10\,m chunks} \\
\cmidrule(lr){2-3}\cmidrule(l){4-6}
Variant & Mean$\downarrow$ & F@10$\uparrow$ & Err.$\downarrow$ & P@3$\uparrow$ & R@3$\uparrow$ \\
\midrule
\grp{OpenVINS poses}
\ours DAVIO mapper, graph      & 0.087 & 0.78 & 0.040 & 61.9 & 52.9 \\
\ours DAVIO mapper, poses fixed & 0.105 & 0.70 & 0.040 & 62.3 & 52.7 \\
\quad + ScaRF windows          & 0.101 & 0.69 & 0.047 & 61.4 & 44.7 \\
\quad + DA3-Large              & 0.093 & 0.73 & 0.038 & 73.0 & 57.5 \\
ScaRF mapper                   & 0.084 & 0.69 & 0.043 & 61.6 & 43.9 \\
\midrule
\grp{Reference poses}
\ours DAVIO mapper, graph or fixed & 0.069 & 0.88 & 0.041 & 67.8 & 54.7 \\
\quad + ScaRF windows          & 0.069 & 0.82 & 0.048 & 62.8 & 43.5 \\
ScaRF mapper                   & 0.040 & 0.89 & 0.029 & 70.6 & 47.7 \\
\bottomrule
\end{tabular}

==> tables/tab_scarf_context.tex <==
% published rows: review/scarf_published_source.json (arXiv:2606.00307v1 Table III); measured rows: this paper
\begin{tabular}{lcccc}\toprule
Method & Seq. & Err. (m) & P@3 (\%) & R@3 (\%)\\\midrule
Scal3R (Offline) & 5/5 & 0.0555 & 53.8 & 44.1\\
DA3-Long & 5/5 & 0.0470 & 56.6 & 51.4\\
MASt3R-SLAM & 4/5 & 0.0410 & 61.4 & 47.8\\
MASt3R-Fusion & 5/5 & 0.0582 & 54.4 & 41.8\\
VGGT-SLAM2 & 5/5 & 0.1686 & 23.8 & 21.9\\
VGGT(D)-SLAM2 & 5/5 & 0.0409 & 60.6 & 50.1\\
ScaRF w/o pose input & 5/5 & 0.0218 & 79.5 & 54.3\\
ScaRF-SLAM & 5/5 & 0.0199 & 81.3 & 55.8\\
\midrule
DAVIO online, DA3-Base & 5/5 & 0.0444 & 60.8 & 38.8\\
DAVIO online, DA3-Large & 5/5 & 0.0327 & 71.9 & 38.3\\
DAVIO mapper offline, fixed, DA3-Large & 5/5 & 0.0377 & 73.0 & 57.5\\
ScaRF mapper, DA3-Base, our poses & 5/5 & 0.0429 & 61.6 & 43.9\\
\bottomrule\end{tabular}

